Can Pre-trained Vision and Language Models Answer Visual Information-Seeking Questions?

Pre-trained vision and language models have demonstrated state-of-the-art capabilities over existing tasks involving images and texts, including visual question answering. However, it remains unclear whether these models possess the capability to answer questions that are not only querying visual content but knowledge-intensive and information-seeking. In this study, we introduce InfoSeek, a visual question answering dataset tailored for information-seeking questions that cannot be answered with only common sense knowledge. Using InfoSeek, we analyze various pre-trained visual question answering models and gain insights into their characteristics. Our findings reveal that state-of-the-art pre-trained multi-modal models (e.g., PaLI-X, BLIP2, etc.) face challenges in answering visual information-seeking questions, but fine-tuning on the InfoSeek dataset elicits models to use fine-grained knowledge that was learned during their pre-training. Furthermore, we show that accurate visual entity recognition can be used to improve performance on InfoSeek by retrieving relevant documents, showing a significant space for improvement.

==> sections/ethical.tex <==
We employ 30 full-time, in-house annotators to collect questions and answers. These annotators are adults and native English speakers residing in the U.S. They are fully aware of the research purpose behind the data collection.
To ensure fair compensation for their time and effort, we pay each annotator \$17.8 per hour, which exceeds the minimum wage in the U.S.
We take measures to ensure the content shown to the annotators is not distressing, and they have the freedom to skip any task that makes them uncomfortable.
The annotation task has received approval from the internal committee.
\ourdataset comprises existing open-sourced images sourced from image recognition and image retrieval datasets, and we adhere to the corresponding terms of usage for academic research purposes.
The original answer texts are sourced from publicly available resources such as Wikipedia and Wikidata.

We believe this study sheds light on how visual-language models can assist people with real-world use cases by answering queries related to visual information seeking. We hope this research will encourage the benchmarking of pre-trained visual language models in their ability to handle knowledge-intensive questions regarding visual information, similar to the way current large language models are benchmarked on TriviaQA~\citep{joshi-etal-2017-triviaqa}.
Furthermore, we believe our analysis on existing visual-language models could provide insights into the future development of multi-modal instruction fine-tuning and raise consideration of taking answer distribution granularity into the instruction prompt design.

==> tables_and_figures/figure_infoseek_examples.tex <==
\begin{figure*}[ht!]
  \centering
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm]{assets/infoseek_images/sport.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: Who is the founder of this sport?}
      \item \footnotesize \textsf{\textbf{A}: Kanō Jigorō}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/bird.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the length of this bird in centimetre?}
      \item \footnotesize \textsf{\textbf{A}: 120-170}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/equipment.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: Who is the inventor of this object?}
      \item \footnotesize \textsf{\textbf{A}: James Gregory}
    \end{itemize}
  \end{minipage}
  \vspace{0.5cm} % Adjust the vertical space as needed
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/dog.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the country of origin of this animal?}
      \item \footnotesize \textsf{\textbf{A}: Rhodesia}
    \end{itemize}
  \end{minipage}
  \vspace{0.5cm} % Adjust the vertical space as needed
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/building3.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: In which year did this building officially open?}
      \item \footnotesize \textsf{\textbf{A}: 1930}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/food.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: Which year was this food invented?}
      \item \footnotesize \textsf{\textbf{A}: 1935}
    \end{itemize}
  \end{minipage}
%   \begin{minipage}[t]{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth,height=2.7cm]{assets/infoseek_images/lake.png}
%     \begin{itemize}[nosep, align=left, leftmargin=*]
%       \item \footnotesize \textbf{Q}: Which mountain range does this lake belong to?
%       \item \footnotesize \textbf{A}: Alp
%     \end{itemize}
%   \end{minipage}
    \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/piano.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the highest note this item can play?}
      \item \footnotesize \textsf{\textbf{A}: C8}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/plant.png}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: Where is this plant native to?}
      \item \footnotesize \textsf{\textbf{A}: Ecuador}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/airplane1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the cruise speed of this aircraft (kilometer per hour)?}
      \item \footnotesize \textsf{\textbf{A}: 828}
    \end{itemize}
  \end{minipage}
  \vspace{0.5cm} % Adjust the vertical space as needed
    \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/animal1.JPEG}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: Which country is this animal endemic to?
}
      \item \footnotesize \textsf{\textbf{A}: Madagascar}
    \end{itemize}
  \end{minipage}
      \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/bird1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: How heavy does this bird typically grow up to in terms of gram?
}
      \item \footnotesize \textsf{\textbf{A}: 4.3}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/bridge1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: Who is the structure engineer of this bridge?
}
      \item \footnotesize \textsf{\textbf{A}: Hellmut Homberg}
    \end{itemize}
  \end{minipage}
 
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/mountain1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What country does this mountain belong to?
}
      \item \footnotesize \textsf{\textbf{A}: North Macedonia}
    \end{itemize}
  \end{minipage}
  \vspace{0.5cm} % Adjust the vertical space as needed
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/lake1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the area in square kilometers of this lake?
}
      \item \footnotesize \textsf{\textbf{A}: 29.8}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/fish1.JPEG}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is this fish named after?
}
      \item \footnotesize \textsf{\textbf{A}: lemon}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/insect1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the closest parent taxonomy of this insect?
}
      \item \footnotesize \textsf{\textbf{A}: Asterocampa}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/plant1.JPEG}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the basionym of this plant?
}
      \item \footnotesize \textsf{\textbf{A}: Agaricus sect. Lepiota}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/car1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: What is the manufacturer of this vehicle?
}
      \item \footnotesize \textsf{\textbf{A}: Suzuki}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/building1.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: Who does this place commemorate?
}
      \item \footnotesize \textsf{\textbf{A}: Mohammad Ali Jinnah}
    \end{itemize}
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
        \begin{tikzpicture}
        \node [inner sep=0pt] at (0,0) {\includegraphics[width=\linewidth,height=2.7cm ]{assets/infoseek_images/building2.jpg}};
        \draw [white, rounded corners=\ClipSep, line width=\ClipSep] 
            (current bounding box.north west) -- 
            (current bounding box.north east) --
            (current bounding box.south east) --
            (current bounding box.south west) -- cycle
            ;
    \end{tikzpicture}
    \begin{itemize}[nosep, align=left, leftmargin=*]
      \item \footnotesize \textsf{\textbf{Q}: In which year was this building built?
}
      \item \footnotesize \textsf{\textbf{A}: 1661}
    \end{itemize}
  \end{minipage}
  \vspace{1cm} 
  \caption{Random examples from the training set of \infoseek$_\text{Wikidata}$.}
  \vspace{0.5cm} 
  \label{fig:infoseek_examples}
\end{figure*}

==> tables_and_figures/table_result_zeroshot.tex <==
\begin{table}[!htbp]
\centering
\small
\tabcolsep 6pt
\begin{tabular}{lcc}
\toprule
\textbf{Model} & $\textbf{\ourdataset}_{\text{Wikidata}}$ & $\textbf{\ourdataset}_{\text{Human}}$\\
\midrule
PaLI-17B &  2.0 & 1.7\\
PaLI-X & 2.0 & 1.6 \\
InstructBLIP & 7.4 & 7.2\\
BLIP2 & \textbf{11.3} & \textbf{8.6}\\
\bottomrule
\end{tabular}
\caption{Zero-shot Performance. change to bar chart and add after finetuning performance improvement.}
\label{tab:zeroshot}
%  \vspace{-10pt}
\end{table}
